A Minimax Approach Against Multi-Armed Adversarial Attacks Detection

Multi-armed adversarial attacks, in which multiple algorithms and objective loss functions are simultaneously used at evaluation time, have been shown to be highly successful in fooling state-of-the-art adversarial examples detectors while requiring no specific side information about the detection mechanism. By formalizing the problem at hand, we can propose a solution that aggregates the soft-probability outputs of multiple pre-trained detectors according to a minimax approach. The proposed framework is mathematically sound, easy to implement, and modular, allowing for integrating existing or future detectors. Through extensive evaluation on popular datasets (e.g., CIFAR10 and SVHN), we show that our aggregation consistently outperforms individual state-of-the-art detectors against multi-armed adversarial attacks, making it an effective solution to improve the resilience of available methods.

==> plots/sota.tex <==
\begin{figure}[t]
	\centering
		\begin{subfigure}[b]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{plots/auroc.png}
		\vspace{-1.5\baselineskip}
		\caption{Analysis \auc}
		\label{fig:sota_auroc}
	\end{subfigure}
		\begin{subfigure}[b]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{plots/fpr.png}
		\vspace{-1.5\baselineskip}
		\caption{Analysis  \fpr}
		\label{fig:sota_fpr}
	\end{subfigure}
	\caption{SOTA's performances under {\mead} grouped by norm. The plots reflects the results of Tabs. 5-8 in~\cite{GranesePRMP2022ECMLPKDD}. We focus on the best supervised method (i.e., NSS~\cite{NSS}) and the best unsupervised method (i.e., FS~\cite{FS}).}
	\label{fig:sota}
\end{figure}

==> tables/sota.tex <==
\begin{table*}[!htbp]
\centering
\caption{Simultaneous attacks detection: SOTA comparison on CIFAR10. The supervised methods are trained on natural and adversarial examples created with PGD algorithm, perturbation magnitude $0.03125$ and L$_\infty$ norm constraint. We include in our investigation both supervised (NSS~\cite{NSS}, KD-BU~\cite{KDBU}, LID~\cite{LID}) and unsupervised (FS~\cite{FS}, MagNet~\cite{MagNet}). We indicate in \textbf{bold} the best results and we highlight in \textcolor{gray}{gray} the column corresponding to the best method.}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{r|aa|cc|cc||cc|cc}
\toprule
 %&
  %\multicolumn{12}{c}{\textbf{NSS}} \Bstrut \\ \cline{2-13} &
  & 
  \multicolumn{2}{c|}{NSS} & \multicolumn{2}{c|}{KD-BU}& \multicolumn{2}{c||}{LID}& \multicolumn{2}{c|}{FS} &
  \multicolumn{2}{c}{MagNet} %&   \multicolumn{2}{c}{0.5}
  \Tstrut\Bstrut \\ \cmidrule{2-11} 
  &
  \auc &
  \fpr &
  \auc &
  \fpr &
  \auc &
  \fpr &
  \auc &
  \fpr &
  \auc &
  \fpr  \\
  \cmidrule{2-11}
  \textbf{Norm L$_1$}\\\textcolor{gray}{PGD1}\\
  $\varepsilon$ = 5 &
9
  \midrule
  
  %%%%%%%%%%%% Norm 2
  
 \textbf{Norm L$_2$} \\ \textcolor{gray}{PGD2}\\

  $\varepsilon$ = 0.125 &
{48.3} & 94.3 &
{42.0} & 96.6 &
{61.3} & 90.6 &
{\textbf{67.5}} & \textbf{77.4} &
{43.1} & 96.9
 \\
$\varepsilon$ = 0.25 &
{53.2} & 91.2 &
{38.4} & 96.8 &
{47.9} & 96.5 &
{\textbf{75.9}} & \textbf{66.1} &
{47.3} & 95.4
 \\
$\varepsilon$ = 0.3125 &
{55.8} & 89.2 &
{38.6} & 96.8 &
{49.7} & 95.8 &
{\textbf{77.0}} & \textbf{64.1} &
{48.7} & 94.8
 \\
$\varepsilon$ = 0.5 &
{63.3} & 82.6 &
{47.9} & 96.2 &
{47.6} & 97.9 &
{\textbf{77.6}} & \textbf{61.4} &
{50.6} & 93.8
 \\
$\varepsilon$ = 1 &
{\textbf{76.4}} & 67.5 &
{74.2} & 92.1 &
{65.2} & 84.1 &
{74.7} & \textbf{65.0} &
{53.0} & 90.1
 \\
$\varepsilon$ = 1.5 &
{\textbf{81.0}} & 63.0 &
{80.1} & 90.1 &
{77.0} & \textbf{56.2} &
{74.5} & 65.1 &
{55.3} & 88.3
 \\
$\varepsilon$ = 2 &
{\textbf{82.6}} & 62.3 &
{81.3} & 89.7 &
{81.5} & \textbf{46.4} &
{73.7} & 65.2 &
{56.9} & 88.2
 \\
   
  
%   %%%%%%%%%%%%
  \textcolor{gray}{DeepFool} \\ 
No $\varepsilon$ & 
{57.0} & 91.7 &
{67.1} & 94.0 &
{\textbf{70.9}} & 86.9 &
{66.0} & \textbf{78.2} &
{51.1} & 94.7
\Bstrut \\ 

  \textcolor{gray}{CW2} \\ 
$\varepsilon$ = 0.01 &
{56.4} & 90.8 &
{53.0} & 95.1 &
{61.6} & 92.5 & 
{\textbf{86.7}} & \textbf{46.3} &
{50.5} & 94.7
\Bstrut \\ 

  \textcolor{gray}{HOP}   \\ 
$\varepsilon$ = 0.1 &
{66.1} & 87.0 &
{67.3} & 94.0 &
{72.2} & 83.6 &
{\textbf{75.7}} & \textbf{69.0} &
{52.2} & 93.8 
\Bstrut \\ \midrule
  
%   %%%%%% Infinite norm

 \textbf{Norm L$_\infty$} \\ \textcolor{gray}{PGDi, FGSM, BIM}\\

  $\varepsilon$ = 0.03125 &
{\textbf{83.0}} & 55.3 &
{29.2} & 97.3 &
{41.4} & 96.5 &
{59.6} & 79.0 &
{58.6} & 82.0
 \\
$\varepsilon$ = 0.0625 &
{\textbf{96.0}} & \textbf{17.2} &
{35.2} & 96.9 &
{58.4} & 83.9 &
{53.7} & 80.3 &
{74.6} & 51.2
 \\
$\varepsilon$ = 0.25 &
{\textbf{97.3}} & \textbf{0.6} &
{45.1} & 96.4 &
{58.0} & 89.5 &
{49.4} & 83.2 &
{97.0} & 5.2
 \\
$\varepsilon$ = 0.5 &
{82.5} & 100.0 &
{43.1} & 96.6 &
{58.6} & 86.7 &
{54.1} & 78.8 &
{\textbf{98.0}} & \textbf{3.5}
 \\

 %   %%%%%%%

  \textcolor{gray}{PGDi, FGSM, BIM, SA} \\ 
$\varepsilon$ = 0.125 &
{9.4} & 99.9 &
{34.9} & 97.0 &
{56.7} & 91.8 &
{46.5} & 86.3 &
{\textbf{87.0}} & \textbf{40.0}
 \\
%   %%%%%%%
  
 \textcolor{gray}{PGDi, FGSM, BIM, CWi} \\ 
$\varepsilon$ = 0.3125 &
{\textbf{63.2}} & 99.1 &
{33.2} & 97.1 &
{49.5} & 96.1 &
{52.7} & \textbf{79.3} &
{52.6} & 94.5
\Bstrut \\ \midrule
  
  %%%%%%%%%%%%% No norm
  \textbf{No norm} \\ \textcolor{gray}{STA}\\

No $\varepsilon$ &
{\textbf{88.5}} & \textbf{38.8} &
{65.4} & 94.2 &
{88.0} & 58.1 & 
{62.7} & 82.5 &
{79.9} & 45.7
\Bstrut \\ 
\hline
\midrule
Average overall the attacks
&
{\textbf{71.8}} & \textbf{66.1} &
{53.0} & 95.2 &
{64.0} & 81.8 &
{66.4} & 73.6 &
{64.6} &  69.7\\
  \bottomrule
\end{tabular}
}
\label{tab:sota}
\end{table*}


